Learning to Hash with Binary Deep Neural Network

This work proposes deep network models and learning algorithms for unsupervised and supervised binary hashing. Our novel network design constrains one hidden layer to directly output the binary codes. This addresses a challenging issue in some previous works: optimizing non-smooth objective functions due to binarization. Moreover, we incorporate independence and balance properties in the direct and strict forms in the learning. Furthermore, we include similarity preserving property in our objective function. Our resulting optimization with these binary, independence, and balance constraints is difficult to solve. We propose to attack it with alternating optimization and careful relaxation. Experimental results on three benchmark datasets show that our proposed methods compare favorably with the state of the art.

==> experiment_supervise.tex <==
\vspace{-0.2cm}
\section{Evaluation of Supervised Hashing with Binary Deep Neural Network}
\label{sec:eva_SH-BDNN}
This section evaluates the proposed SH-BDNN and compares it with following state-of-the-art supervised hashing methods: Supervised Discrete Hashing (SDH)~\cite{Shen_2015_CVPR}, ITQ-CCA~\cite{DBLP:conf/cvpr/GongL11}, Kernel-based Supervised Hashing (KSH)~\cite{CVPR12:Hashing}, Binary Reconstructive Embedding (BRE)~\cite{Kulis_learningto}. For all compared methods, we use the implementation and the suggested parameters provided by the authors.
\vspace{-0.2cm}
\subsection{Dataset, evaluation protocol, and implementation note}
\subsubsection{Dataset} We evaluate and compare methods on CIFAR-10 and MNIST datasets. The descriptions of these datasets are presented in section~\ref{subsec:data-imp-eva}.

\vspace{-0.4cm} 
\subsubsection{Evaluation protocol} Follow the literature~\cite{Shen_2015_CVPR,DBLP:conf/cvpr/GongL11,CVPR12:Hashing}, we report the retrieval results in two metrics: 1) mean Average Precision (mAP) and 2) precision of Hamming radius $2$ (precision$@2$).

\vspace{-0.4cm}
\subsubsection{Implementation note} The network configuration is same as UH-BDNN excepting the final layer is removed. The values of parameters $\lambda_1$, $\lambda_2$, $\lambda_3$ and $\lambda_4$ are empirically set using cross validation as $10^{-3}$, $5$, $1$ and $10^{-4}$, respectively. The max iteration number $T$ is empirically set to 5. 

Follow the settings in ITQ-CCA~\cite{DBLP:conf/cvpr/GongL11}, SDH~\cite{Shen_2015_CVPR},  all training samples are used in the learning for these two methods. For SH-BDNN, KSH~\cite{CVPR12:Hashing} and BRE~\cite{Kulis_learningto} where label information is leveraged by the pairwise label matrix, we randomly select $3,000$ training samples from each class and use %these selected samples
them for learning. The ground truths of queries are defined by the class labels from the datasets.

\vspace{-0.1cm}
\subsection{Retrieval results}
\begin{figure*}[!t]
\vspace{-1em}
\centering
\subfigure[CIFAR10]{
       \includegraphics[scale=0.32]{BDNN_cifar10_mapK_sup_8-16-24-32.pdf}
       \label{fig:cifar_mAP_sup}
}
\subfigure[MNIST]{
       \includegraphics[scale=0.32]{BDNN_mnist_mapK_sup_8-16-24-32.pdf} 
       \label{fig:mnist_mAP_sup}
}
\caption[]{mAP comparison between SH-BDNN and state-of-the-art supervised hashing methods on CIFAR10 and MNIST.}
\label{fig:cifar10_mnist_sup}
\end{figure*}
\begin{table}[!t]
   \centering
   \footnotesize
   \caption{Precision at Hamming distance $r=2$ comparison between SH-BDNN and state-of-the-art supervised hashing methods on CIFAR10 and MNIST.}
    \begin{tabular}{|l|c| c| c| c|c| c| c| c|}
		\hline
	  \multirow{2}{*}{} & \multicolumn{4}{|c|}{CIFAR10} & \multicolumn{4}{|c|}{MNIST} \\
\cline{1-9}	$L$    		          &8 &16 &24 &32    		    &8 &16 &24 &32     \\ \hline 
SH-BDNN						      &54.12 &67.32 &69.36 &69.62   &84.26 &94.67 &94.69 &95.51 
		\\ \hline
SDH\cite{Shen_2015_CVPR} 		  &31.60 &62.23 &67.65 &67.63   &36.49  &93.00 &93.98 &94.43 
		\\ \hline  
%ITQ-CCA\cite{DBLP:conf/cvpr/GongL11}&49.14 &67.68 &69.47 &69.19 &54.35 &79.99 &84.12 &84.57
ITQ-CCA\cite{DBLP:conf/cvpr/GongL11}&49.14 &65.68 &67.47 &67.19  &54.35 &79.99 &84.12 &84.57
		\\ \hline		                                  
KSH\cite{CVPR12:Hashing}		  &44.81 &64.08 &67.01 &65.76   &68.07  &90.79 &92.86 &92.41  
		\\ \hline
BRE\cite{Kulis_learningto}        &23.84 &41.11 &47.98 &44.89   &37.67  &69.80 &83.24 &84.61
		\\ \hline
	  \end{tabular}
	  \label{tab:soa-sup-cifar10-mnist-pre}
	  \vspace{-0.2cm}
\end{table}
%Fig.~\ref{fig:cifar10_mnist_sup} and Table~\ref{tab:soa-sup-cifar10-mnist-pre} show comparative results on CIFAR10 and MNIST datasets. 
On CIFAR10 dataset, Fig.~\ref{fig:cifar_mAP_sup} and Table~\ref{tab:soa-sup-cifar10-mnist-pre} clearly show the proposed SH-BDNN outperforms all compared methods by a fair margin at all code lengths in both mAP and precision@2. %The most competitive method to SH-BDNN is CCA-ITQ~\cite{DBLP:conf/cvpr/GongL11}. 

%The gains of SH-BDNN over the current state-of-the-art SDH~\cite{Shen_2015_CVPR} are \textbf{+17\%}, \textbf{+3.1\%}, \textbf{+4.9\%} and \textbf{+3.4\%} at 8, 16, 32 and 64 bits, respectively. The gains of SH-BDNN over KSH~\cite{CVPR12:Hashing} which also uses pairwise label matrix are \textbf{+7.6\%}, \textbf{+6.2\%}, \textbf{+5.9\%} and \textbf{+5.3\%} at 8, 16, 32 and 64 bits, respectively. In term of precision$@r$, the proposed SH-BDNN clearly outperforms the compared methods at low code lengths, i.e., $L = 8,16$. SDH~\cite{Shen_2015_CVPR} becomes comparable with SH-BDNN when increasing the code lengths, i.e., $L=32, 64$.

On MNIST dataset, Fig.~\ref{fig:mnist_mAP_sup} and Table~\ref{tab:soa-sup-cifar10-mnist-pre} show the proposed SH-BDNN significant outperforms the current state-of-the-art SDH at low code length, i.e., $L=8$. When $L$ increases, SH-BDNN and SDH~\cite{Shen_2015_CVPR} achieve similar performance. SH-BDNN significantly outperforms remaining methods, i.e. KSH~\cite{CVPR12:Hashing}, ITQ-CCA~\cite{DBLP:conf/cvpr/GongL11}, BRE~\cite{Kulis_learningto} in both mAP and precision@2.

\paragraph{Comparison with CNN-based hashing~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}}
We compare our proposed SH-BDNN to very recent CNN-based supervised hashing methods~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}. %In~\cite{DBLP:conf/aaai/XiaPLLY14}, the author propose CNNH, a supervised hashing method in which the learning is decomposed into two separate steps. First step is the learning of hash codes from the supervised information. Second step is the simultaneously learning hash functions and image representations based on the learned hash codes. 
In~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}, the authors propose the  framework in which the image features and hash codes are simultaneously learned by combining CNN layers and binary quantization layer into a large model. As mentioned in~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}, those works achieve good performance because of (i) the power of CNN layers in capturing discriminative features from the input image and (ii) the joint learning of features and hash codes. Note that our work is different from those works, i.e., our work is about hash function/hash codes learning with given features, while those works are simultaneously image features and hash codes learning. To make a fair comparison to those works, we follow the comparison setting in~\cite{DBLP:journals/tip/ZhangLZZZ15}. In~\cite{DBLP:journals/tip/ZhangLZZZ15}, when comparing their CNN-based hashing method to other non CNN-based hashing methods, the authors use AlexNet features~\cite{jia2014caffe} as input for other methods. Hence, we use AlexNet features as input to our model when comparing our proposed method to~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}. We set up the experiments on CIFAR10 similar to~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15} for a fair comparison. In~\cite{DBLP:conf/cvpr/LaiPLY15}, the query set contains 1K images (100 images per class) randomly sampled from the dataset; the rest 59K images are used as database for retrieval; the training set contains 5K images (500 images per class) randomly sampled from that 59K images. In~\cite{DBLP:journals/tip/ZhangLZZZ15}, the query set contains 10K images (1K images per class) randomly sampled from the dataset; the rest 50K image are used as the training set; %Note that, we use less than 50K images, i.e. we randomly sample only 30K images from that 50K, for training our model in comparison to~\cite{DBLP:journals/tip/ZhangLZZZ15}. 
in testing step, each query image is searched within the query set itself by applying the leave-one-out procedure.

We compare our SH-BDNN to ~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15} in term of mAP because only the numbers on mAP are clearly showed in~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}. The comparative mAP are shown in Table~\ref{tab:soa-sup-cvpr15-tip}. Table~\ref{tab:soa-sup-cvpr15-tip} clearly shows that at the same code length, the proposed SH-BDNN outperforms both~\cite{DBLP:conf/cvpr/LaiPLY15} and~\cite{DBLP:journals/tip/ZhangLZZZ15}.
\begin{table}[!t]
   \centering
   \footnotesize
   \caption{comparative mAP between proposed SH-BDNN and CNN-based supervised hashing~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15}. The results of~\cite{DBLP:conf/cvpr/LaiPLY15,DBLP:journals/tip/ZhangLZZZ15} are directly cited from the corresponding papers.}
    \begin{tabular}{|c|c|c|c||c|c| c| c|}
%		\hline
%				$L$	   		    &24    &32  &48      &$L$      &24     &32    &48 \\ \hline 
%SH-BDNN						    &57.30 &58.66 &60.08 &SH-BDNN  &68.81  &69.66 &71.01 
%		\\ \hline
%\cite{DBLP:conf/cvpr/LaiPLY15}  &56.60 &55.80 &58.10 &\cite{DBLP:journals/tip/ZhangLZZZ15} &62.19  &62.87 &63.05 \\ \hline  
		\hline
				$L$	   		    &24    &32  &48      &$L$      &24     &32    &48 \\ \hline 
SH-BDNN						    &57.30 &58.66 &60.08 &SH-BDNN  &65.21  &66.22 &66.53 
		\\ \hline
\cite{DBLP:conf/cvpr/LaiPLY15}  &56.60 &55.80 &58.10 &\cite{DBLP:journals/tip/ZhangLZZZ15} &62.19  &62.87 &63.05 \\ \hline  
	  \end{tabular}
	  \label{tab:soa-sup-cvpr15-tip}
	  \vspace{-0.2cm}
\end{table}

==> experiment_supervise_v2_copy.tex <==
\vspace{-0.4cm}
\section{Evaluation of Supervised Hashing with Binary Deep Neural Network (SH-BDNN)}
\label{sec:eva_SH-BDNN}
\vspace{-0.2cm}
This section evaluates the proposed SH-BDNN and compares it with following state-of-the-art supervised hashing methods: Supervised Discrete Hashing (SDH)~\cite{Shen_2015_CVPR}, ITQ-CCA~\cite{DBLP:conf/cvpr/GongL11}, Kernel-based Supervised Hashing (KSH)~\cite{CVPR12:Hashing}, Binary Reconstructive Embedding (BRE)~\cite{Kulis_learningto}. For all compared methods, we use the implementation and the suggested parameters provided by the authors.
\vspace{-0.2cm}
\subsection{Dataset, evaluation protocol, and implementation note}
\subsubsection{Dataset} We evaluate and compare methods on CIFAR-10 and MNIST datasets. The descriptions of these datasets are presented in section~\ref{subsec:data-imp-eva}.

\vspace{-0.4cm} 
\subsubsection{Evaluation protocol} Follow the literature~\cite{Shen_2015_CVPR,DBLP:conf/cvpr/GongL11,CVPR12:Hashing}, we report the retrieval results in two metrics: 1) mean Average Precision (mAP) and 2) precision of Hamming radius $2$ (precision$@2$).

\vspace{-0.4cm}
\subsubsection{Implementation note} The network configuration is same as UH-BDNN excepting the final layer is removed. The values of parameters $\lambda_1$, $\lambda_2$, $\lambda_3$ and $\lambda_4$ are empirically set using cross validation as $10^{-3}$, $5$, $1$ and $10^{-4}$, respectively. The max iteration number $T$ is empirically set to 5. 

Follow the settings in ITQ-CCA~\cite{DBLP:conf/cvpr/GongL11}, SDH~\cite{Shen_2015_CVPR},  all training samples are used in the learning for these two methods. For SH-BDNN, KSH~\cite{CVPR12:Hashing} and BRE~\cite{Kulis_learningto} where label information is leveraged by the pairwise label matrix, we randomly select $3,000$ training samples from each class and use %these selected samples
them for learning. The ground truths of queries are defined by the class labels from the datasets.

\vspace{-0.3cm}
\subsection{Retrieval results}
\begin{figure*}[!t]
\vspace{-1em}
\centering
\subfigure[CIFAR10]{
       \includegraphics[scale=0.30]{BDNN_cifar10_mapK_sup_8-16-24-32.pdf}
       \label{fig:cifar_mAP_sup}
}
\subfigure[MNIST]{
       \includegraphics[scale=0.30]{BDNN_mnist_mapK_sup_8-16-24-32.pdf} 
       \label{fig:mnist_mAP_sup}
}
\vspace{-0.2cm}
\caption[]{mAP comparison between SH-BDNN and state-of-the-art supervised hashing methods on CIFAR10 and MNIST.}
\label{fig:cifar10_mnist_sup}
\end{figure*}
\begin{table}[!t]
   \centering
   \footnotesize
   \caption{Precision at Hamming distance $r=2$ comparison between SH-BDNN and state-of-the-art supervised hashing methods on CIFAR10 and MNIST.}
    \begin{tabular}{|l|c| c| c| c|c| c| c| c|}
		\hline
	  \multirow{2}{*}{} & \multicolumn{4}{|c|}{CIFAR10} & \multicolumn{4}{|c|}{MNIST} \\
\cline{1-9}	$L$    		          &8 &16 &24 &32    		    &8 &16 &24 &32     \\ \hline 
SH-BDNN						      &54.12 &67.32 &69.36 &69.62   &84.26 &94.67 &94.69 &95.51 
		\\ \hline
SDH\cite{Shen_2015_CVPR} 		  &31.60 &62.23 &67.65 &67.63   &36.49  &93.00 &93.98 &94.43 
		\\ \hline  
%ITQ-CCA\cite{DBLP:conf/cvpr/GongL11}&49.14 &67.68 &69.47 &69.19 &54.35 &79.99 &84.12 &84.57
ITQ-CCA\cite{DBLP:conf/cvpr/GongL11}&49.14 &65.68 &67.47 &67.19  &54.35 &79.99 &84.12 &84.57
		\\ \hline		                                  
KSH\cite{CVPR12:Hashing}		  &44.81 &64.08 &67.01 &65.76   &68.07  &90.79 &92.86 &92.41  
		\\ \hline
BRE\cite{Kulis_learningto}        &23.84 &41.11 &47.98 &44.89   &37.67  &69.80 &83.24 &84.61
		\\ \hline
	  \end{tabular}
	  \label{tab:soa-sup-cifar10-mnist-pre}
	  \vspace{-0.2cm}
\end{table}
%Fig.~\ref{fig:cifar10_mnist_sup} and Table~\ref{tab:soa-sup-cifar10-mnist-pre} show comparative results on CIFAR10 and MNIST datasets. 
On CIFAR10 dataset, Fig.~\ref{fig:cifar_mAP_sup} and Table~\ref{tab:soa-sup-cifar10-mnist-pre} clearly show the proposed SH-BDNN outperforms all compared methods by a fair margin at all code lengths in both mAP and precision@2. %The most competitive method to SH-BDNN is CCA-ITQ~\cite{DBLP:conf/cvpr/GongL11}. 

%The gains of SH-BDNN over the current state-of-the-art SDH~\cite{Shen_2015_CVPR} are \textbf{+17\%}, \textbf{+3.1\%}, \textbf{+4.9\%} and \textbf{+3.4\%} at 8, 16, 32 and 64 bits, respectively. The gains of SH-BDNN over KSH~\cite{CVPR12:Hashing} which also uses pairwise label matrix are \textbf{+7.6\%}, \textbf{+6.2\%}, \textbf{+5.9\%} and \textbf{+5.3\%} at 8, 16, 32 and 64 bits, respectively. In term of precision$@r$, the proposed SH-BDNN clearly outperforms the compared methods at low code lengths, i.e., $L = 8,16$. SDH~\cite{Shen_2015_CVPR} becomes comparable with SH-BDNN when increasing the code lengths, i.e., $L=32, 64$.

On MNIST dataset, Fig.~\ref{fig:mnist_mAP_sup} and Table~\ref{tab:soa-sup-cifar10-mnist-pre} show the proposed SH-BDNN significantly outperforms the current state-of-the-art SDH at low code length, i.e., $L=8$. When $L$ increases, SH-BDNN and SDH~\cite{Shen_2015_CVPR} achieve similar performance. In comparison to remaining methods, i.e., KSH~\cite{CVPR12:Hashing}, ITQ-CCA~\cite{DBLP:conf/cvpr/GongL11}, BRE~\cite{Kulis_learningto}, SH-BDNN outperforms these methods by a large margin in both mAP and precision@2.\\
%\vspace{-0.3cm}
%\paragraph{Comparison with CNN-based hashing methods~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}}
\textit{Comparison with CNN-based hashing methods~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}} 
We also compare our proposed SH-BDNN to very recent CNN-based supervised hashing methods, i.e., Deep Semantic Ranking Hashing (DSRH)~\cite{DBLP:conf/cvpr/ZhaoHWT15} and Deep Regularized Similarity Comparison Hashing (DRSCH)~\cite{DBLP:journals/tip/ZhangLZZZ15}. %In~\cite{DBLP:conf/aaai/XiaPLLY14}, the author propose CNNH, a supervised hashing method in which the learning is decomposed into two separate steps. First step is the learning of hash codes from the supervised information. Second step is the simultaneously learning hash functions and image representations based on the learned hash codes. 
In~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}, the authors propose the  framework in which the image features and hash codes are simultaneously learned by combining CNN layers and binary mapping layer into a model. %As mentioned in~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}, those works achieve good performance because of (i) the power of CNN layers in capturing discriminative features from the input image and (ii) the joint learning of image features and hash codes. 
%Note that our work is different from those works, i.e., our work focuses on hash codes learning with given image features, while those works are simultaneously image features and hash codes learning. 
It is worth noting that after getting CNN features from the top layers (i.e., fully connected layers) of CNNs, the binary mapping layer in~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15} only applies a simple operation, i.e., an approximation of $sgn$ function (i.e., $logistic$~\cite{DBLP:conf/cvpr/ZhaoHWT15}, $tanh$~\cite{DBLP:journals/tip/ZhangLZZZ15}), on CNN features for achieving the approximated binary codes. 
Our SH-BDNN advances~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15} in the way to map the image features to the binary codes. Given the image features (i.e., pre-trained CNN features), %in order to achieve the binary codes, 
we apply multiple transformations on these features; we constrain one layer to directly output the binary code, without involving $sgn$ function. Furthermore, our learned codes ensure good properties, i.e. independence and balance, while DRSCH~\cite{DBLP:journals/tip/ZhangLZZZ15} does not consider such properties, and DSRH~\cite{DBLP:conf/cvpr/ZhaoHWT15} only considers the balance of codes. 

To make a fair comparison to~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}, we follow the comparison setting in those works. In~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}, when comparing their CNN-based hashing to other non CNN-based hashing methods, the authors use pre-trained CNN features (e.g. AlexNet features~\cite{jia2014caffe}) as input for other methods. Follow that setting, we use AlexNet features as input for SH-BDNN  
when comparing SH-BDNN to~\cite{DBLP:conf/cvpr/ZhaoHWT15,DBLP:journals/tip/ZhangLZZZ15}. We set up the experiments on CIFAR10 similar to~\cite{DBLP:journals/tip/ZhangLZZZ15}, i.e., the query set contains 10K images (1K images per class) randomly sampled from the dataset; the rest 50K image are used as the training set; %Note that, we use less than 50K images, i.e. we randomly sample only 30K images from that 50K, for training our model in comparison to~\cite{DBLP:journals/tip/ZhangLZZZ15}. 
in the testing step, each query image is searched within the query set itself by applying the leave-one-out procedure.

%We present the comparative results in term of mAP because only the numbers on mAP are clearly showed in~\cite{DBLP:journals/tip/ZhangLZZZ15}. The comparative mAP, presented in Table~\ref{tab:soa-sup-cvpr15-tip}, clearly shows that at the same code length, the proposed SH-BDNN outperforms both~\cite{DBLP:conf/cvpr/ZhaoHWT15} and~\cite{DBLP:journals/tip/ZhangLZZZ15}.
%\begin{table}[!t]
%   \centering
%   \footnotesize
%   \caption{comparative mAP between proposed SH-BDNN and CNN-based supervised hashing DSRH~\cite{DBLP:conf/cvpr/ZhaoHWT15} and DRSCH~\cite{DBLP:journals/tip/ZhangLZZZ15}. The results of DSRH and DRSCH are directly cited from~\cite{DBLP:journals/tip/ZhangLZZZ15}.}
%    \begin{tabular}{|c|@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|}
%		\hline
%				$L$	   	                   &16	    &24     &32    &48      \\ \hline 
%SH-BDNN					                   &64.30  &65.21  &66.22 &66.53   \\ \hline
%DSRH\cite{DBLP:conf/cvpr/ZhaoHWT15}        &60.84  &61.08  &61.74 &61.77  \\ \hline
%DRSCH\cite{DBLP:journals/tip/ZhangLZZZ15}  &61.46  &62.19  &62.87 &63.05 \\ \hline  
%	  \end{tabular}
%	  \label{tab:soa-sup-cvpr15-tip}
%	  \vspace{-0.2cm}
%\end{table}
%The comparative results between the proposed SH-BDNN and DSRH~\cite{DBLP:conf/cvpr/ZhaoHWT15}, DRSCH~\cite{DBLP:journals/tip/ZhangLZZZ15} are shown in Table~\ref{tab:soa-sup-cvpr15-tip}. The results clearly show that at the same code length, the proposed SH-BDNN outperforms~\cite{DBLP:conf/cvpr/ZhaoHWT15} and~\cite{DBLP:journals/tip/ZhangLZZZ15} in both mAP and precision@2.
The comparative results between the proposed SH-BDNN and DSRH~\cite{DBLP:conf/cvpr/ZhaoHWT15}, DRSCH~\cite{DBLP:journals/tip/ZhangLZZZ15}, presented in Table~\ref{tab:soa-sup-cvpr15-tip}, clearly show that at the same code length, the proposed SH-BDNN outperforms~\cite{DBLP:conf/cvpr/ZhaoHWT15} and~\cite{DBLP:journals/tip/ZhangLZZZ15} in both mAP and precision@2.
\begin{table}[!t]
   \centering
   \footnotesize
   \vspace{-0.2em}
   \caption{Comparison between SH-BDNN and CNN-based hashing DSRH~\cite{DBLP:conf/cvpr/ZhaoHWT15}, DRSCH~\cite{DBLP:journals/tip/ZhangLZZZ15} on CIFAR10. The results of DSRH and DRSCH are cited from~\cite{DBLP:journals/tip/ZhangLZZZ15}.}
   \vspace{-0.2em}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline
	  \multirow{2}{*}{} & \multicolumn{4}{|c|}{mAP} & \multicolumn{4}{|c|}{precison@2} \\
\cline{1-9}	$L$    		          &16 &24 &32 &48    		  &16 &24 &32 &48     \\ \hline 
%SH-BDNN				&64.30 &65.21 &66.22 &66.53   &59.87 &62.67 &62.80 &62.42 \\ \hline
SH-BDNN				&64.30 &65.21 &66.22 &66.53   &56.87 &58.67 &58.80 &58.42 \\ \hline
DRSCH\cite{DBLP:journals/tip/ZhangLZZZ15}&61.46 &62.19 &62.87 &63.05 &52.34 &53.07 &52.31 &52.03\\ \hline  
DSRH\cite{DBLP:conf/cvpr/ZhaoHWT15}&60.84 &61.08 &61.74 &61.77 &50.36 &52.45 &50.37 &49.38\\ \hline
	  \end{tabular}
	  \label{tab:soa-sup-cvpr15-tip}
	  \vspace{-0.4cm}
\end{table}

==> related_work.tex <==
\section{Related Work}

